Autonomous Human-Robot Interaction via Operator Imitation

Teleoperated robotic characters can perform expressive interactions with humans, relying on the operators' experience and social intuition. In this work, we propose to create autonomous interactive robots, by training a model to imitate operator data. Our model is trained on a dataset of human-robot interactions, where an expert operator is asked to vary the interactions and mood of the robot, while the operator commands as well as the pose of the human and robot are recorded. Our approach learns to predict continuous operator commands through a diffusion process and discrete commands through a classifier, all unified within a single transformer architecture. We evaluate the resulting model in simulation and with a user study on the real system. We show that our method enables simple autonomous human-robot interactions that are comparable to the expert-operator baseline, and that users can recognize the different robot moods as generated by our model. Finally, we demonstrate a zero-shot transfer of our model onto a different robotic platform with the same operator interface.

==> sections/figures/qual.tex <==
\begin{figure*}[t!]
 % \vspace{-2mm}
 \centering
  \begin{minipage}{\linewidth}
  \centering
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={600 150 200 200},clip]{sections/figures/angry/angry_1.png}
   \\ 
  \end{minipage}
  % \begin{minipage}{0.24\linewidth}
  %  \centering
  %  \includegraphics[width=\linewidth,trim={600 150 200 200},clip]{sections/figures/angry/angry_2.pdf}
  %  \\ 
  % \end{minipage}~
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={600 150 200 200},clip]{sections/figures/angry/angry_2.png}
   \\ 
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={600 150 200 200},clip]{sections/figures/angry/angry_3.png}
   \\ 
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={600 150 200 200},clip]{sections/figures/angry/angry_4.png}
   \\ 
  \end{minipage}
 \end{minipage}
 \\~\\ \vspace{0mm}
   \small{Angry Mood}
    \\~\\ \vspace{0mm}
  \begin{minipage}{\linewidth}
  \centering
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={700 200 200 100},clip]{sections/figures/sad/sad_1.png}
   \\ 
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={700 200 200 100},clip]{sections/figures/sad/sad_3.png}
   \\ 
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={700 200 200 100},clip]{sections/figures/sad/sad_4.png}
   \\ 
  \end{minipage}
  \begin{minipage}{0.24\linewidth}
   \centering
   \includegraphics[width=\linewidth,trim={700 200 200 100},clip]{sections/figures/sad/sad_5.png}
   \\ 
  \end{minipage}
  \end{minipage}
  \\~\\ \vspace{0mm}
   \small{Sad Mood}
 \caption{\textbf{Example behavior of different moods.} In the angry mood, the robot refuses interactions and steps away from the human (top). In the sad mood, the robot turns away from the human, has its head tilted towards the ground and occasionally shakes its head (bottom).}
 \label{fig:qual}
\end{figure*}

% The happy policy imitates a jump after a human has performed a jump.
